Representation Of Lexical Stylistic Features In Language Models' Embedding Space

The representation space of pretrained Language Models (LMs) encodes rich information about words and their relationships (e.g., similarity, hypernymy, polysemy) as well as abstract semantic notions (e.g., intensity). In this paper, we demonstrate that lexical stylistic notions such as complexity, formality, and figurativeness, can also be identified in this space. We show that it is possible to derive a vector representation for each of these stylistic notions from only a small number of seed pairs. Using these vectors, we can characterize new texts in terms of these dimensions by performing simple calculations in the corresponding embedding space. We conduct experiments on five datasets and find that static embeddings encode these features more accurately at the level of words and phrases, whereas contextualized LMs perform better on sentences. The lower performance of contextualized representations at the word level is partially attributable to the anisotropy of their vector space, which can be corrected to some extent using techniques like standardization.

==> fables/tab_isotropy_layeragg.tex <==
% \begin{table*}[!t]
%     \centering
%     \scalebox{0.8}{

%     \begin{tabular}{ll|cc|cc|c}
%     \toprule
%         \textbf{Pooling} & \textbf{Model} & \multicolumn{2}{c|}{\textbf{Complexity}} & \multicolumn{2}{c|}{\textbf{Formality}} & \textbf{Figurativeness} \\
%         ~ & ~ & short & long & short & long & long \\
%          \hline
%         \multirow{5}{1.5cm}{Mean} & static & 84.8 & 60.0 & \textbf{76.8} & 82.8 & 54.3 \\ 

%         \hline
%         \multirow{5}{1.5cm}{Max} & static & 89.4 & 58.0 & 76.0 & 63.4 & 56.0 \\ 

%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance of three anisotropy reduction methods (all-but-the-top/standardization/rank-based) under the \textbf{layer aggregation} setting. The highest performance within each pooling method (Mean/Max) is in boldface.}
%     \label{table:isotropy_layeragg}
% \end{table*}
